Queue management for slo-oriented large language model serving

Large language model (LLM) serving is becoming an increasingly critical workload for cloud providers. Existing LLM serving systems focus on interactive requests, such as chatbots and coding assistants, with tight latency SLO requirements. However, when such systems execute batch requests that have relaxed SLOs along with interactive requests, it leads to poor multiplexing and inefficient resource utilization. To address these challenges, we propose QLM, a queue management system for LLM serving. QLM maintains batch and interactive requests across different models and SLOs in a request queue. Optimal ordering of the request queue is critical to maintain SLOs while ensuring high resource utilization. To generate this optimal ordering, QLM uses a Request Waiting Time (RWT) Estimator that estimates the waiting times for requests in the request queue. These estimates are used by a global scheduler to orchestrate LLM Serving Operations (LSOs) such as request pulling, request eviction, load balancing, and model swapping. Evaluation on heterogeneous GPU devices and models with real-world LLM serving dataset shows that QLM improves SLO attainment by 40-90% and throughput by 20-400% while maintaining or improving device utilization compared to other state-of-the-art LLM serving systems. QLM's evaluation is based on the production requirements of a cloud provider. QLM is publicly available at https://www.github.com/QLM-project/QLM.

==> 0000-intro_v3.tex <==
\section{Introduction}
\label{s:introduction}

% Why is queueing a problem? current queues cannot handle it, why use LSOs with queues? why merge LSOs with queuing


\begin{figure}[!tb]
    \centering
    \includegraphics[width=\linewidth]{resources/QLM_motivation.pdf}
    \caption{Scenarios for workload consolidation in LLM serving systems.}
    \label{fig:scenarios}
\end{figure}


\BLUE{\noindent \textbf{Motivation.} 
The emergence of large language models (LLMs) such as OpenAI GPT-4 and Google Gemini has enabled a wide range of novel AI applications~\cite{compound-ai-blog,bommasani2021opportunities,wu2023autogen}, including chatbots and coding assistants.
Consequently, serving LLMs has become an increasingly critical workload, catering to both enterprise and consumer applications with service-level objectives (SLOs)~\cite{jyothi2016morpheus,qiu2020firm,wang2024efficient}.

Recent work on LLM serving has primarily focused on interactive services, which have strict SLO requirements for inter-token latency and time-to-first token.
In production systems, in addition to these interactive services, there is also a growing need to support batch LLM queries, which are required for tasks such as data wrangling, log processing, and model fine-tuning.
These batch LLM queries have much higher SLO values, ranging from minutes to hours, as they do not require immediate execution.
There is an opportunity for workload consolidation by jointly serving batch and interactive requests to maximize device utilization and reduce the total resource requirement.

Specifically, we identify the following workload consolidation scenarios as shown in Figure~\ref{fig:scenarios}:
\begin{enumerate}[wide=0pt, label=(\alph*)]
    \item \emph{Batch and Interactive Request Co-location}: Instead of using separate LLM serving instances for batch and interactive requests, they can be co-located on a single LLM serving instance.
    A major challenge that arises with such co-location is that interactive requests may need to wait at the front of the waiting queue before execution on the LLM serving instance, causing head-of-line (HOL) blocking. To prevent such HOL blocking, an alternative strategy is to evict existing batch requests from the LLM serving instance and put them back into the waiting queue. This effectively allows interactive requests to be executed immediately in a nearly isolated manner. 
    Compared to traditional DNN serving systems, request eviction in LLM serving requires saving the state, i.e. the KV cache or output tokens to minimize throughput disruption for the batch requests.
    
    \item \emph{Multi-model Batch Request Co-location:} Instead of using multiple LLM serving instances for each model, the same serving instance could be used with the models being swapped in and out on demand. However, as LLMs are much larger compared to DNN models, the swap times are also much larger ( for e.g. $\sim$20s for a 70B parameter model).
    Consequently, serving requests in their order of arrival for multiple models can lead to repeated model swapping and loss in throughput.
    Instead, \emph{requests groups} can be created per model, and this grouping reduces required model swaps and minimize loss in throughput. 
\end{enumerate}

Both of these scenarios require the management of a \emph{global request queue} that comprise a mix of interactive and batch requests with multiple models.
Previous work on LLM serving~\cite{kwon2023efficient,yu2022orca,tensorrt,tgi,aiops2024qiu,li2023alpaserve,sheng2023flexgen,wu2023fast} has largely focused on interactive requests where maintaining global queues is unnecessary, as it would lead to violation of strict request latency requirements.
For example, Lluminix~\cite{llumnix} autoscales and adds new LLM serving instances when the queue size exceeds a threshold.
However, when the workload comprises of a combination of batch and interactive requests, maintaining request queues can be beneficial as it presents opportunities for resource savings while still adhering to latency requirements, as discussed in the two scenarios above.

% \begin{figure}[t]
%     \hspace{-3ex}
%     \centering
%     \begin{minipage}{.1\textwidth}
%         \centering
%         \includegraphics{resources/results/Intro_diagram_HOL_blocking.pdf}
%         \label{fig:Predictable Waiting Time}
%     \end{minipage}%
%     \hspace{11ex}
%     $\vpointer$
%     \centering
%     \begin{minipage}{.2\textwidth}
%     \centering
%     \includegraphics{resources/results/Intro_diagram_latency.pdf}
%     \label{fig:swaping_with_reordering}
%     \end{minipage}%
%     \hfill
%     \vspace{-20pt}
%     \caption{\sysname nearly eliminates HOL blocking time in both single and multi-model serving scenarios and enables SLO attainment for batch and latency-sensitive applications. }
%     \label{fig:intro_result}
% \end{figure}

% -> why waiting time???
% However, serving LLMs can be surprisingly resource-intensive and costly.
% For example, a single A100 GPU is only able to serve $<$1 request per second for a medium-sized model with 13 billion parameters.
% State-of-the-art LLM serving systems such as vLLM~\cite{kwon2023efficient}, Orca~\cite{yu2022orca}, and TensorRT-LLM~\cite{tensorrt} improve serving throughput by upto 20$\times$ over traditional ML serving systems with novel techniques such as \emph{continuous batching}~\cite{yu2022orca} and \emph{paged attention}~\cite{kwon2023efficient}.
% (e.g., with \textit{continuous batching}~\cite{yu2022orca} and \textit{PagedAttention}~\cite{kwon2023efficient})


%LLM serving systems have HOL blocking problem,
%QLM introduces LSOs and optimizes them for 
\noindent
\textbf{Our Contributions.}
% Achieving end-to-end latency SLOs together with throughput and utilization goals is challenging.
% To address this problem, we introduce \sysname, a queue management framework for SLO-oriented LLM serving.
We present \sysname, a system for workload consolidation in LLM serving that manages the global request queue to minimize the total resource usage while maximizing SLO satisfaction.
\sysname leverages three major ideas in its queue management framework:
\begin{enumerate}[wide=4pt,label=(\alph*)]
\item \emph{Request Group Abstraction:}
\sysname uses \emph{request groups}, where requests that share the same performance characteristics (i.e. model and latency SLO) are grouped together and decisions are taken per request group instead of per request.
Decision making at the per-request group level offers two advantages: 
\begin{enumerate*}
    \item Request groups are a natural abstraction for scenarios such as multi-model swapping (shown in Scenario 1), and
    \item Requests groups improve system scalability by reducing the overhead of decision making. 
\end{enumerate*}
\sysname places these request groups in virtual queues that determine the order in which requests are consumed by the LLM serving instances.

\item \emph{Request Waiting Time (RWT) Estimator:}
When making decisions on order in requests groups, it is beneficial to estimate queue waiting time to ensure that SLOs are met.
However, estimating the waiting time is challenging because the execution time for a request depends on its output token length, which is unknown apriori before executing the request~\cite{kwon2023efficient} (i.e., stochastic in nature).
We observe and mathematically prove that despite these stochastic effects, the waiting time in LLM serving is predictable and provide an estimator for it.

\item \emph{Global Scheduler:}
Finally, \sysname uses a \emph{Global Scheduler} (described in Section~\ref{s:plan_generation}) that leverages the waiting time estimates of request groups to create an optimal ordering and assignment of request groups onto the virtual queues to maximize SLO attainment.
\end{enumerate}


\noindent \textbf{Results.}
We demonstrate \sysname on vLLM~\cite{kwon2023efficient} as the backend LLM-serving system.
\sysname uses the following four basic LLM Serving Operations (LSOs) to manage the request queue (see \cref{s:lso} for details):
\begin{enumerate*}[label=(\arabic*)]
\item \emph{Request Pulling} from the global waiting queue into the running batch in the GPU,
\item \emph{Request Eviction} from the running batch back into the waiting queue,
\item \emph{Model Swapping} from CPU to GPU memory, and
\item \emph{Load Balancing} across multiple LLM model instances.
\end{enumerate*}

We evaluate \sysname on three popular LLMs of varying sizes (i.e., Mistral-7B~\cite{mistral}, Vicuna-13B~\cite{vicuna}, and Llama-70B~\cite{touvron2023llama}) on heterogeneous GPU clusters with NVIDIA A10 and A100 GPUs.
We adopt workloads from a real-world LLM dataset: ShareGPT~\cite{shareGPT} using setups derived from our production requirements.
Our experiments demonstrate the following major improvements with \sysname:
\begin{enumerate}[wide=0pt,label=(\arabic*)]
    \item \emph{SLO Attainment:} \sysname achieves 40--90\% higher SLO attainment compared to the vanilla vLLM serving system and 50--90\% higher SLO attainment compared to traditional ML serving systems like SHEPHERD,
    \item \emph{Request Throughput:} \sysname improves the request throughput in a multi-model serving system by 400\% on average and in a single-model serving system by 20\% on average compared to other LLM serving systems, and
    \item \emph{LSO Ablation Study:} \sysname demonstrates that all LSOs contribute to SLO attainment and throughput improvement.
    Notably, we find that model warm start improves throughput by 300\% in multi-model serving, and request eviction improves SLO attainment by 80\% in single-model serving.
\end{enumerate}
}
% \noindent
% \textbf{Putting \sysname in Perspective.}
% In production LLM serving, it is critical to support effective multi-model queue management and scale to a large number of LLMs~\cite{hu2021lora,sheng2023slora} with varying SLO requirements and request rates while ensuring high throughput and device utilization.
% % \hq{Effective queue management is the key to multi-model LLM serving, which often confronts the significant challenge of device shortage and queue accumulation but device under-utilization, from our experience as a major cloud provider offering ML-as-a-Service.}
% \sysname is the first queue management framework that enforces the end-to-end latency SLOs while improving LLM-serving throughput and device utilization by systematically orchestrating backend LSOs.
% % (1) existing LLM serving frameworks that ignore SLOs are already covered in the intro
% % (2) existing SLO-aware model serving frameworks
% Previous frameworks do not apply to LLMs because the per-request execution time is variable and nondeterministic, which, combined with continuous batching behavior, affects the decision-making for each LSO.
% Andes~\cite{liu2024andes} defines Quality-of-Experience (QoE) for LLM serving as token delivery speed and proposes a preemptive scheduler that maximizes QoE.
% However, Andes does not enforce the end-to-end latency SLO, only optimizes for one LSO (e.g., request preemption), and negatively impacts system throughput by up to 10\%.




% 1. Reordering of queue based on a queue abstraction …..
%     1. Some of these are distributions …. Based on Bayes estimator (how is profiling done for these? Using this data, which is to minimize uncertainty and determine distribution of key parameters, how are these parameters decided you can talk later)
% 2. If there are distributions, then each is modeled with a This paper investigates SLO and LSO based-modeling because in the end SLO is the decided parameter that the customer demand, and no method uses it as the central parameter of optimization, while there are SLO-based parameters for model serving they lack this

% Our model serving is based on addressing 3 key challenges: 1. How best to optimize the queue? (a) continuous reprioirtizng queue entries to achieve what? Optimal queue length for the highest priority job.. there are uncertainty in the model serving parameters that can be handled with bayesian stats using profiling data for such and such… 3. using stochastic programming,2.  bayesian model gives you the distribution for chosen parameters: waiting time and completion time main uncertainties based on profiling data from 


% The major parameter of the queue total completion time and waiting time, these are stochastic they are not deterministic and we determine these disitrbutions with profiling to build a Bayesian model to determine the best estimates for these two distributions. And our results are so much better…. Doesnt take into account uncertainty, no reordering, 


% SLOs are the prime metric and no one uses these in the most effective way and purpose of this paper as an SLO-driven model parameters, put those results at the beginning, even though there are other SLO-based approaches we are better because….. 1. 2. 3.  That are indeed the inadequacies of the previous work….. handling uncertainty and no way… they do normal optimization which as we show is insufficient, to achieve….


% Make connection of the previous work….. here are the issues of the previous work…. You dont have to say this is how we address it…. 


% By not doing dynamic reordering they are stuck 

% Role of the SLO in deciding priority per-user, in the process we see significant uncertainty is in the wait time and overall execution time, we go to the data

% Contributions of this work are:

% While determining this SLO, now with the SLO these SLOs can be highly variable and introduce, now we have uncertainty under control we can use stochastic programming,


% Need to determine key parameters because you have talked about queue parameters previously - mean based analysis how much worse can you get?

%separate paragraph: service is not quantized, dont assume 
%explanation of cascading effect
%promotes continual chance that request will meet its SLO, second benefit is that service times are stochastic, benefit of being stochastic previous people assume it to be constant which is based on a few samples, mean value approach doesnt take into account variance of the distribution and the only way to do that is to get full posterior using Bayesian
%now that you have distribution you use a stochastic solver (give detailed results)
%you can maintain higher throughput but you will be missing many SLO deadlines, need to make distributon of service times (whatever the metric is)
